A Unified Evaluation Framework for Novelty Detection and Accommodation in NLP with an Instantiation in Authorship Attribution

State-of-the-art natural language processing models have been shown to achieve remarkable performance in 'closed-world' settings where all the labels in the evaluation set are known at training time. However, in real-world settings, 'novel' instances that do not belong to any known class are often observed. This renders the ability to deal with novelties crucial. To initiate a systematic research in this important area of 'dealing with novelties', we introduce 'NoveltyTask', a multi-stage task to evaluate a system's performance on pipelined novelty 'detection' and 'accommodation' tasks. We provide mathematical formulation of NoveltyTask and instantiate it with the authorship attribution task that pertains to identifying the correct author of a given text. We use Amazon reviews corpus and compile a large dataset (consisting of 250k instances across 200 authors/labels) for NoveltyTask. We conduct comprehensive experiments and explore several baseline methods for the task. Our results show that the methods achieve considerably low performance making the task challenging and leaving sufficient room for improvement. Finally, we believe our work will encourage research in this underexplored area of dealing with novelties, an important step en route to developing robust systems.

==> Tables/ds1_sample_class_detection.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}
    {
\begin{tabular}{lllllllll}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Novelties \\ Predicted\end{tabular}}} & \multicolumn{4}{l}{\textbf{\# of classes detected}}                                & \multicolumn{4}{l}{\textbf{\# of Samples detected}}           \\ \cline{2-9} 
                                                                                          & \textbf{CM} & \textbf{ED} & \textbf{MD} & \multicolumn{1}{l|}{\textbf{MP}} & \textbf{CM} & \textbf{ED} & \textbf{MD} & \textbf{MP} \\ \hline
\multicolumn{1}{l}{\textbf{1000}}                                                        & 95             & 10             & 100            & \multicolumn{1}{l|}{100}            & 337            & 866            & 910            & 873            \\
\multicolumn{1}{l}{\textbf{2000}}                                                        & 100            & 15             & 100            & \multicolumn{1}{l|}{100}            & 777            & 1375           & 1766           & 1738           \\
\multicolumn{1}{l}{\textbf{3000}}                                                        & 100            & 22             & 100            & \multicolumn{1}{l|}{100}            & 1242           & 1941           & 2621           & 2559           \\
\multicolumn{1}{l}{\textbf{4000}}                                                        & 100            & 25             & 100            & \multicolumn{1}{l|}{100}            & 1740           & 2333           & 3447           & 3365           \\
\multicolumn{1}{l}{\textbf{5000}}                                                        & 100            & 27             & 100            & \multicolumn{1}{l|}{100}            & 2261           & 2700           & 4230           & 4146           \\
\multicolumn{1}{l}{\textbf{6000}}                                                        & 100            & 33             & 100            & \multicolumn{1}{l|}{100}            & 2802           & 3195           & 5046           & 4932           \\
\multicolumn{1}{l}{\textbf{7000}}                                                        & 100            & 37             & 100            & \multicolumn{1}{l|}{100}            & 3330           & 3563           & 5717           & 5671           \\
\multicolumn{1}{l}{\textbf{8000}}                                                        & 100            & 42             & 100            & \multicolumn{1}{l|}{100}            & 3872           & 4157           & 6280           & 6407           \\
\multicolumn{1}{l}{\textbf{9000}}                                                        & 100            & 47             & 100            & \multicolumn{1}{l|}{100}            & 4401           & 4567           & 6869           & 7151           \\
\multicolumn{1}{l}{\textbf{10000}}                                                       & 100            & 52             & 100            & \multicolumn{1}{l|}{100}            & 4974           & 5198           & 7410           & 7818           \\ \hline
\end{tabular}
}
\caption{
    insert caption
    }
    \label{tab7}
\end{table}

==> Tables/ds1_stage1_combined.tex <==
\begin{table*}[t!]
    \centering
    \small
    \resizebox{\linewidth}{!}
    {
        \begin{tabular}{llllllllll}
\hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}\# of \\ Novelties\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Known \\ Class\\ precision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Known\\ class \\ recall\end{tabular}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Known \\ Class\\ F1\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Novel\\ Class \\ Precision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Novel\\ Class\\ Recall\end{tabular}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Novel \\ Class \\ F1\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Overall\\ Precision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Overall\\ Recall\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Overall\\ F1\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\textbf{2000}}                                                       & 47.95                                                                       & 74.60                                                                    & \multicolumn{1}{l|}{58.38}                                                                & 38.85                                                                       & 7.77                                                                    & \multicolumn{1}{l|}{12.95}                                                                 & 47.86                                                                & 73.94                                                             & 58.11                                                         \\
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 47.49                                                                       & 65.56                                                                    & \multicolumn{1}{l|}{55.08}                                                                & 43.50                                                                       & 17.40                                                                   & \multicolumn{1}{l|}{24.86}                                                                 & 47.45                                                                & 65.08                                                             & 54.88                                                         \\
\multicolumn{1}{l|}{\textbf{6000}}                                                       & 47.61                                                                       & 57.54                                                                    & \multicolumn{1}{l|}{52.11}                                                                & 46.70                                                                       & 28.02                                                                   & \multicolumn{1}{l|}{35.03}                                                                 & 47.60                                                                & 57.25                                                             & 51.98                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 48.12                                                                       & 49.97                                                                    & \multicolumn{1}{l|}{49.03}                                                                & 48.40                                                                       & 38.72                                                                   & \multicolumn{1}{l|}{43.02}                                                                 & 48.12                                                                & 49.86                                                             & 48.97                                                         \\
\multicolumn{1}{l|}{\textbf{10000}}                                                      & 49.06                                                                       & 42.64                                                                    & \multicolumn{1}{l|}{45.63}                                                                & 49.74                                                                       & 49.74                                                                   & \multicolumn{1}{l|}{49.74}                                                                 & 49.07                                                                & 42.71                                                             & 45.67                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 50.48                                                                       & 35.40                                                                    & \multicolumn{1}{l|}{41.62}                                                                & 50.64                                                                       & 60.77                                                                   & \multicolumn{1}{l|}{55.25}                                                                 & 50.49                                                                & 35.65                                                             & 41.79                                                         \\
\multicolumn{1}{l|}{\textbf{14000}}                                                      & 52.95                                                                       & 28.10                                                                    & \multicolumn{1}{l|}{36.72}                                                                & 51.37                                                                       & 71.92                                                                   & \multicolumn{1}{l|}{59.93}                                                                 & 52.93                                                                & 28.53                                                             & 37.08                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 56.07                                                                       & 20.03                                                                    & \multicolumn{1}{l|}{29.52}                                                                & 51.62                                                                       & 82.60                                                                   & \multicolumn{1}{l|}{63.54}                                                                 & 56.03                                                                & 20.65                                                             & 30.18                                                         \\
\multicolumn{1}{l|}{\textbf{18000}}                                                      & 61.48                                                                       & 11.10                                                                    & \multicolumn{1}{l|}{18.80}                                                                & 51.34                                                                       & 92.41                                                                   & \multicolumn{1}{l|}{66.01}                                                                 & 61.38                                                                & 11.91                                                             & 19.95                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Compute Mean}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{\textbf{2000}}                                                       & 48.91                                                                       & 79.87                                                                    & \multicolumn{1}{l|}{60.67}                                                                & 68.75                                                                       & 13.75                                                                   & \multicolumn{1}{l|}{22.92}                                                                 & 49.11                                                                & 79.22                                                             & 60.63                                                         \\
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 45.56                                                                       & 71.13                                                                    & \multicolumn{1}{l|}{55.54}                                                                & 58.33                                                                       & 23.33                                                                   & \multicolumn{1}{l|}{33.33}                                                                 & 45.69                                                                & 70.66                                                             & 55.50                                                         \\
\multicolumn{1}{l|}{\textbf{6000}}                                                       & 41.65                                                                       & 61.56                                                                    & \multicolumn{1}{l|}{49.68}                                                                & 53.25                                                                       & 31.95                                                                   & \multicolumn{1}{l|}{39.94}                                                                 & 41.77                                                                & 61.27                                                             & 49.67                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 36.91                                                                       & 52.62                                                                    & \multicolumn{1}{l|}{43.39}                                                                & 51.96                                                                       & 41.57                                                                   & \multicolumn{1}{l|}{46.19}                                                                 & 37.06                                                                & 52.51                                                             & 43.45                                                         \\
\multicolumn{1}{l|}{\textbf{10000}}                                                      & 32.44                                                                       & 43.78                                                                    & \multicolumn{1}{l|}{37.27}                                                                & 51.98                                                                       & 51.98                                                                   & \multicolumn{1}{l|}{51.98}                                                                 & 32.63                                                                & 43.86                                                             & 37.42                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 27.91                                                                       & 35.83                                                                    & \multicolumn{1}{l|}{31.38}                                                                & 52.27                                                                       & 62.73                                                                   & \multicolumn{1}{l|}{57.03}                                                                 & 28.15                                                                & 36.10                                                             & 31.63                                                         \\
\multicolumn{1}{l|}{\textbf{14000}}                                                      & 24.95                                                                       & 28.26                                                                    & \multicolumn{1}{l|}{26.50}                                                                & 52.44                                                                       & 73.41                                                                   & \multicolumn{1}{l|}{61.17}                                                                 & 25.22                                                                & 28.71                                                             & 26.85                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 20.47                                                                       & 20.57                                                                    & \multicolumn{1}{l|}{20.52}                                                                & 52.52                                                                       & 84.03                                                                   & \multicolumn{1}{l|}{64.64}                                                                 & 20.79                                                                & 21.20                                                             & 20.99                                                         \\
\multicolumn{1}{l|}{\textbf{18000}}                                                      & 12.59                                                                       & 10.05                                                                    & \multicolumn{1}{l|}{11.18}                                                                & 51.37                                                                       & 92.46                                                                   & \multicolumn{1}{l|}{66.04}                                                                 & 12.98                                                                & 10.87                                                             & 11.83                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Compute Euclid Distance}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{l|}{\textbf{2000}}                                                       & 52.69                                                                       & 85.30                                                                    & \multicolumn{1}{l|}{65.14}                                                                & 88.30                                                                       & 17.66                                                                   & \multicolumn{1}{l|}{29.43}                                                                 & 53.04                                                                & 84.63                                                             & 65.21                                                         \\
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 56.77                                                                       & 84.39                                                                    & \multicolumn{1}{l|}{67.88}                                                                & 86.17                                                                       & 34.47                                                                   & \multicolumn{1}{l|}{49.24}                                                                 & 57.06                                                                & 83.90                                                             & 67.92                                                         \\
\multicolumn{1}{l|}{\textbf{6000}}                                                       & 61.80                                                                       & 82.93                                                                    & \multicolumn{1}{l|}{70.82}                                                                & 84.10                                                                       & 50.46                                                                   & \multicolumn{1}{l|}{63.07}                                                                 & 62.02                                                                & 82.61                                                             & 70.85                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 66.59                                                                       & 77.29                                                                    & \multicolumn{1}{l|}{71.54}                                                                & 78.50                                                                       & 62.80                                                                   & \multicolumn{1}{l|}{69.78}                                                                 & 66.71                                                                & 77.15                                                             & 71.55                                                         \\
\multicolumn{1}{l|}{\textbf{10000}}                                                      & 66.03                                                                       & 70.30                                                                    & \multicolumn{1}{l|}{68.10}                                                                & 74.10                                                                       & 74.10                                                                   & \multicolumn{1}{l|}{74.10}                                                                 & 66.11                                                                & 70.34                                                             & 68.16                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 62.80                                                                       & 61.12                                                                    & \multicolumn{1}{l|}{61.95}                                                                & 69.68                                                                       & 83.62                                                                   & \multicolumn{1}{l|}{76.02}                                                                 & 62.87                                                                & 61.34                                                             & 62.10                                                         \\
\multicolumn{1}{l|}{\textbf{14000}}                                                      & 57.14                                                                       & 49.33                                                                    & \multicolumn{1}{l|}{52.95}                                                                & 64.95                                                                       & 90.93                                                                   & \multicolumn{1}{l|}{75.78}                                                                 & 57.22                                                                & 49.74                                                             & 53.22                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 46.65                                                                       & 34.35                                                                    & \multicolumn{1}{l|}{39.57}                                                                & 59.52                                                                       & 95.24                                                                   & \multicolumn{1}{l|}{73.26}                                                                 & 46.78                                                                & 34.95                                                             & 40.01                                                         \\
\multicolumn{1}{l|}{\textbf{18000}}                                                      & 28.30                                                                       & 18.55                                                                    & \multicolumn{1}{l|}{22.41}                                                                & 54.84                                                                       & 98.71                                                                   & \multicolumn{1}{l|}{70.51}                                                                 & 28.56                                                                & 19.34                                                             & 23.06                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Compute Mahalanobis Distance}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{\textbf{2000}}                                                       & 53.72                                                                       & 85.18                                                                    & \multicolumn{1}{l|}{65.89}                                                                & 86.90                                                                       & 17.38                                                                   & \multicolumn{1}{l|}{28.97}                                                                 & 54.05                                                                & 84.51                                                             & 65.93                                                         \\
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 58.58                                                                       & 83.88                                                                    & \multicolumn{1}{l|}{68.98}                                                                & 84.12                                                                       & 33.65                                                                   & \multicolumn{1}{l|}{48.07}                                                                 & 58.83                                                                & 83.38                                                             & 68.99                                                         \\
\multicolumn{1}{l|}{\textbf{6000}}                                                       & 64.06                                                                       & 82.19                                                                    & \multicolumn{1}{l|}{72.00}                                                                & 82.20                                                                       & 49.32                                                                   & \multicolumn{1}{l|}{61.65}                                                                 & 64.24                                                                & 81.86                                                             & 71.99                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 70.61                                                                       & 79.46                                                                    & \multicolumn{1}{l|}{74.77}                                                                & 80.09                                                                       & 64.07                                                                   & \multicolumn{1}{l|}{71.19}                                                                 & 70.70                                                                & 79.31                                                             & 74.76                                                         \\
\multicolumn{1}{l|}{\textbf{10000}}                                                      & 78.35                                                                       & 75.76                                                                    & \multicolumn{1}{l|}{77.03}                                                                & 78.18                                                                       & 78.18                                                                   & \multicolumn{1}{l|}{78.18}                                                                 & 78.34                                                                & 75.78                                                             & 77.04                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 87.24                                                                       & 68.96                                                                    & \multicolumn{1}{l|}{77.03}                                                                & 74.85                                                                       & 89.82                                                                   & \multicolumn{1}{l|}{81.65}                                                                 & 87.12                                                                & 69.17                                                             & 77.11                                                         \\
\multicolumn{1}{l|}{\textbf{14000}}                                                      & 94.42                                                                       & 56.67                                                                    & \multicolumn{1}{l|}{70.83}                                                                & 69.19                                                                       & 96.86                                                                   & \multicolumn{1}{l|}{80.72}                                                                 & 94.18                                                                & 57.07                                                             & 71.07                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 96.40                                                                       & 39.25                                                                    & \multicolumn{1}{l|}{55.79}                                                                & 62.06                                                                       & 99.30                                                                   & \multicolumn{1}{l|}{76.38}                                                                 & 96.06                                                                & 39.84                                                             & 56.32                                                         \\
\multicolumn{1}{l|}{\textbf{18000}}                                                      & 82.84                                                                       & 19.86                                                                    & \multicolumn{1}{l|}{32.04}                                                                & 55.48                                                                       & 99.87                                                                   & \multicolumn{1}{l|}{71.34}                                                                 & 82.57                                                                & 20.65                                                             & 33.04                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Compute Max Probability}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{l|}{\textbf{2000}}                                                       & 51.07                                                                       & 81.63                                                                    & \multicolumn{1}{l|}{62.83}                                                                & 64.70                                                                       & 12.94                                                                   & \multicolumn{1}{l|}{21.57}                                                                 & 51.21                                                                & 80.95                                                             & 62.73                                                         \\
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 55.09                                                                       & 79.28                                                                    & \multicolumn{1}{l|}{65.01}                                                                & 71.50                                                                       & 28.60                                                                   & \multicolumn{1}{l|}{40.86}                                                                 & 55.25                                                                & 78.78                                                             & 64.95                                                         \\
\multicolumn{1}{l|}{\textbf{6000}}                                                       & 60.52                                                                       & 77.81                                                                    & \multicolumn{1}{l|}{68.08}                                                                & 74.67                                                                       & 44.80                                                                   & \multicolumn{1}{l|}{56.00}                                                                 & 60.66                                                                & 77.48                                                             & 68.05                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 67.90                                                                       & 76.66                                                                    & \multicolumn{1}{l|}{72.01}                                                                & 76.89                                                                       & 61.51                                                                   & \multicolumn{1}{l|}{68.34}                                                                 & 67.99                                                                & 76.51                                                             & 72.00                                                         \\
\multicolumn{1}{l|}{\textbf{10000}}                                                      & 77.97                                                                       & 76.10                                                                    & \multicolumn{1}{l|}{77.02}                                                                & 78.74                                                                       & 78.24                                                                   & \multicolumn{1}{l|}{78.49}                                                                 & 77.98                                                                & 76.12                                                             & 77.04                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 71.60                                                                       & 55.78                                                                    & \multicolumn{1}{l|}{62.71}                                                                & 65.45                                                                       & 78.54                                                                   & \multicolumn{1}{l|}{71.40}                                                                 & 71.54                                                                & 56.01                                                             & 62.83                                                         \\
\multicolumn{1}{l|}{\textbf{14000}}                                                      & 62.06                                                                       & 36.95                                                                    & \multicolumn{1}{l|}{46.32}                                                                & 56.86                                                                       & 79.61                                                                   & \multicolumn{1}{l|}{66.34}                                                                 & 62.01                                                                & 37.37                                                             & 46.64                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 50.04                                                                       & 19.35                                                                    & \multicolumn{1}{l|}{27.91}                                                                & 51.10                                                                       & 81.76                                                                   & \multicolumn{1}{l|}{62.89}                                                                 & 50.05                                                                & 19.97                                                             & 28.55                                                         \\
\multicolumn{1}{l|}{\textbf{18000}}                                                      & 30.17                                                                       & 5.54                                                                     & \multicolumn{1}{l|}{9.36}                                                                 & 48.46                                                                       & 87.23                                                                   & \multicolumn{1}{l|}{62.31}                                                                 & 30.35                                                                & 6.35                                                              & 10.50                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Placeholders Algorithm}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{l|}{\textbf{2000}}                                                       & 53.56                                                                       & 83.99                                                                    & \multicolumn{1}{l|}{65.41}                                                                & 82.80                                                                       & 16.56                                                                   & \multicolumn{1}{l|}{27.60}                                                                 & 53.85                                                                & 83.32                                                             & 65.42                                                         \\
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 58.36                                                                       & 82.33                                                                    & \multicolumn{1}{l|}{68.30}                                                                & 82.30                                                                       & 32.92                                                                   & \multicolumn{1}{l|}{47.03}                                                                 & 58.59                                                                & 81.84                                                             & 68.29                                                         \\
\multicolumn{1}{l|}{\textbf{6000}}                                                       & 63.96                                                                       & 80.82                                                                    & \multicolumn{1}{l|}{71.41}                                                                & 82.22                                                                       & 49.33                                                                   & \multicolumn{1}{l|}{61.66}                                                                 & 64.14                                                                & 80.51                                                             & 71.40                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 71.27                                                                       & 79.69                                                                    & \multicolumn{1}{l|}{75.25}                                                                & 81.61                                                                       & 65.29                                                                   & \multicolumn{1}{l|}{72.54}                                                                 & 71.38                                                                & 79.55                                                             & 75.24                                                         \\
\multicolumn{1}{l|}{\textbf{10000}}                                                      & 65.18                                                                       & 64.96                                                                    & \multicolumn{1}{l|}{65.07}                                                                & 69.73                                                                       & 69.73                                                                   & \multicolumn{1}{l|}{69.73}                                                                 & 65.23                                                                & 65.01                                                             & 65.12                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 57.50                                                                       & 48.95                                                                    & \multicolumn{1}{l|}{52.88}                                                                & 61.16                                                                       & 73.39                                                                   & \multicolumn{1}{l|}{66.72}                                                                 & 57.54                                                                & 49.19                                                             & 53.04                                                         \\
\multicolumn{1}{l|}{\textbf{14000}}                                                      & 45.04                                                                       & 35.39                                                                    & \multicolumn{1}{l|}{39.64}                                                                & 56.56                                                                       & 79.18                                                                   & \multicolumn{1}{l|}{65.98}                                                                 & 45.15                                                                & 35.82                                                             & 39.95                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 34.79                                                                       & 23.44                                                                    & \multicolumn{1}{l|}{28.01}                                                                & 53.85                                                                       & 86.16                                                                   & \multicolumn{1}{l|}{66.28}                                                                 & 34.98                                                                & 24.06                                                             & 28.51                                                         \\
\multicolumn{1}{l|}{\textbf{18000}}                                                      & 25.68                                                                       & 12.56                                                                    & \multicolumn{1}{l|}{16.87}                                                                & 52.21                                                                       & 93.97                                                                   & \multicolumn{1}{l|}{67.12}                                                                 & 25.95                                                                & 13.37                                                             & 17.65                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Few shot Open set Recognition}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\end{tabular}
    }
    \caption{ Novelty Detection Stage performance of Dataset 1. 
    }
    \label{tab:ds1_s1}
\end{table*}

==> Tables/ds2_sample_class_detection.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}
    {
\begin{tabular}{lllllllll}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Novelties \\ Predicted\end{tabular}}} & \multicolumn{4}{l}{\textbf{\# of classes detected}}                                & \multicolumn{4}{l}{\textbf{\# of Samples detected}}           \\ \cline{2-9} 
                                                                                          & \textbf{CM} & \textbf{ED} & \textbf{MD} & \multicolumn{1}{l|}{\textbf{MP}} & \textbf{CM} & \textbf{ED} & \textbf{MD} & \textbf{MP} \\ \hline
\multicolumn{1}{l}{\textbf{1000}}                                                        & 55             & 4              & 55             & \multicolumn{1}{l|}{56}             & 310            & 497            & 904            & 874            \\
\multicolumn{1}{l}{\textbf{2000}}                                                        & 55             & 7              & 55             & \multicolumn{1}{l|}{56}             & 657            & 1026           & 1756           & 1723           \\
\multicolumn{1}{l}{\textbf{3000}}                                                        & 55             & 10             & 55             & \multicolumn{1}{l|}{56}             & 1089           & 1799           & 2577           & 2556           \\
\multicolumn{1}{l}{\textbf{4000}}                                                        & 55             & 11             & 55             & \multicolumn{1}{l|}{56}             & 1528           & 1849           & 3376           & 3351           \\
\multicolumn{1}{l}{\textbf{5000}}                                                        & 55             & 13             & 55             & \multicolumn{1}{l|}{56}             & 1984           & 2347           & 4145           & 4111           \\
\multicolumn{1}{l}{\textbf{6000}}                                                        & 55             & 15             & 55             & \multicolumn{1}{l|}{56}             & 2486           & 2802           & 4815           & 4871           \\
\multicolumn{1}{l}{\textbf{7000}}                                                        & 55             & 19             & 55             & \multicolumn{1}{l|}{56}             & 2963           & 3355           & 5377           & 5628           \\
\multicolumn{1}{l}{\textbf{8000}}                                                        & 56             & 21             & 55             & \multicolumn{1}{l|}{56}             & 3472           & 3706           & 5904           & 6340           \\
\multicolumn{1}{l}{\textbf{9000}}                                                        & 56             & 22             & 55             & \multicolumn{1}{l|}{56}             & 3977           & 4002           & 6576           & 7093           \\
\multicolumn{1}{l}{\textbf{10000}}                                                       & 56             & 24             & 55             & \multicolumn{1}{l|}{56}             & 4467           & 4324           & 7010           & 7773           \\ \hline
\end{tabular}
}
\caption{
    insert caption
    }
    \label{tab}
\end{table}

==> Tables/ds2_stage1_combined.tex <==
\begin{table*}[t!]
    \centering
    \small
    \resizebox{\linewidth}{!}
    {
       \begin{tabular}{llllllllll}
\hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}\# of \\ Novelties\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Known \\ Class\\ precision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Known\\ class \\ recall\end{tabular}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Known \\ Class\\ F1\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Novel\\ Class \\ Precision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Novel\\ Class\\ Recall\end{tabular}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Novel \\ Class \\ F1\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Overall\\ Precision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Overall\\ Recall\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Overall\\ F1\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 49.09                                                                       & 76.28                                                                    & \multicolumn{1}{l|}{59.74}                                                                & 37.70                                                                       & 7.54                                                                    & \multicolumn{1}{l|}{12.57}                                                                 & 48.98                                                                & 75.60                                                             & 59.45                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 48.75                                                                       & 67.31                                                                    & \multicolumn{1}{l|}{56.55}                                                                & 43.29                                                                       & 17.32                                                                   & \multicolumn{1}{l|}{24.74}                                                                 & 48.70                                                                & 66.81                                                             & 56.34                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 48.83                                                                       & 58.98                                                                    & \multicolumn{1}{l|}{53.43}                                                                & 46.39                                                                       & 27.84                                                                   & \multicolumn{1}{l|}{34.79}                                                                 & 48.81                                                                & 58.67                                                             & 53.29                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 49.47                                                                       & 51.33                                                                    & \multicolumn{1}{l|}{50.38}                                                                & 48.49                                                                       & 38.79                                                                   & \multicolumn{1}{l|}{43.10}                                                                 & 49.46                                                                & 51.20                                                             & 50.31                                                         \\
\multicolumn{1}{l|}{\textbf{20000}}                                                      & 50.45                                                                       & 43.83                                                                    & \multicolumn{1}{l|}{46.91}                                                                & 49.91                                                                       & 49.91                                                                   & \multicolumn{1}{l|}{49.91}                                                                 & 50.45                                                                & 43.89                                                             & 46.94                                                         \\
\multicolumn{1}{l|}{\textbf{24000}}                                                      & 51.93                                                                       & 36.37                                                                    & \multicolumn{1}{l|}{42.78}                                                                & 50.84                                                                       & 61.01                                                                   & \multicolumn{1}{l|}{55.46}                                                                 & 51.92                                                                & 36.61                                                             & 42.94                                                         \\
\multicolumn{1}{l|}{\textbf{28000}}                                                      & 53.70                                                                       & 28.54                                                                    & \multicolumn{1}{l|}{37.27}                                                                & 51.35                                                                       & 71.89                                                                   & \multicolumn{1}{l|}{59.90}                                                                 & 53.68                                                                & 28.97                                                             & 37.63                                                         \\
\multicolumn{1}{l|}{\textbf{32000}}                                                      & 56.86                                                                       & 20.39                                                                    & \multicolumn{1}{l|}{30.02}                                                                & 51.60                                                                       & 82.56                                                                   & \multicolumn{1}{l|}{63.51}                                                                 & 56.80                                                                & 21.01                                                             & 30.67                                                         \\
\multicolumn{1}{l|}{\textbf{36000}}                                                      & 61.53                                                                       & 11.23                                                                    & \multicolumn{1}{l|}{18.99}                                                                & 51.27                                                                       & 92.29                                                                   & \multicolumn{1}{l|}{65.92}                                                                 & 61.42                                                                & 12.04                                                             & 20.13                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Compute Mean}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 50.07                                                                       & 81.95                                                                    & \multicolumn{1}{l|}{62.16}                                                                & 68.75                                                                       & 13.75                                                                   & \multicolumn{1}{l|}{22.92}                                                                 & 50.25                                                                & 81.27                                                             & 62.10                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 46.41                                                                       & 72.95                                                                    & \multicolumn{1}{l|}{56.73}                                                                & 58.27                                                                       & 23.31                                                                   & \multicolumn{1}{l|}{33.30}                                                                 & 46.52                                                                & 72.46                                                             & 56.66                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 42.47                                                                       & 63.27                                                                    & \multicolumn{1}{l|}{50.82}                                                                & 53.26                                                                       & 31.95                                                                   & \multicolumn{1}{l|}{39.94}                                                                 & 42.58                                                                & 62.95                                                             & 50.80                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 37.63                                                                       & 54.12                                                                    & \multicolumn{1}{l|}{44.39}                                                                & 51.98                                                                       & 41.59                                                                   & \multicolumn{1}{l|}{46.21}                                                                 & 37.77                                                                & 53.99                                                             & 44.45                                                         \\
\multicolumn{1}{l|}{\textbf{20000}}                                                      & 33.38                                                                       & 45.37                                                                    & \multicolumn{1}{l|}{38.46}                                                                & 51.99                                                                       & 51.99                                                                   & \multicolumn{1}{l|}{51.99}                                                                 & 33.57                                                                & 45.43                                                             & 38.61                                                         \\
\multicolumn{1}{l|}{\textbf{24000}}                                                      & 28.75                                                                       & 37.42                                                                    & \multicolumn{1}{l|}{32.52}                                                                & 52.28                                                                       & 62.74                                                                   & \multicolumn{1}{l|}{57.04}                                                                 & 28.98                                                                & 37.68                                                             & 32.76                                                         \\
\multicolumn{1}{l|}{\textbf{28000}}                                                      & 25.77                                                                       & 29.65                                                                    & \multicolumn{1}{l|}{27.57}                                                                & 52.42                                                                       & 73.39                                                                   & \multicolumn{1}{l|}{61.16}                                                                 & 26.03                                                                & 30.08                                                             & 27.91                                                         \\
\multicolumn{1}{l|}{\textbf{32000}}                                                      & 20.81                                                                       & 21.51                                                                    & \multicolumn{1}{l|}{21.15}                                                                & 52.52                                                                       & 84.03                                                                   & \multicolumn{1}{l|}{64.64}                                                                 & 21.12                                                                & 22.13                                                             & 21.61                                                         \\
\multicolumn{1}{l|}{\textbf{36000}}                                                      & 12.80                                                                       & 10.84                                                                    & \multicolumn{1}{l|}{11.74}                                                                & 51.38                                                                       & 92.48                                                                   & \multicolumn{1}{l|}{66.06}                                                                 & 13.19                                                                & 11.65                                                             & 12.37                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Compute Euclid Distance}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 54.01                                                                       & 87.43                                                                    & \multicolumn{1}{l|}{66.77}                                                                & 90.35                                                                       & 18.07                                                                   & \multicolumn{1}{l|}{30.12}                                                                 & 54.37                                                                & 86.74                                                             & 66.84                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 58.14                                                                       & 86.56                                                                    & \multicolumn{1}{l|}{69.56}                                                                & 88.29                                                                       & 35.31                                                                   & \multicolumn{1}{l|}{50.45}                                                                 & 58.44                                                                & 86.05                                                             & 69.61                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 63.11                                                                       & 84.86                                                                    & \multicolumn{1}{l|}{72.39}                                                                & 85.72                                                                       & 51.44                                                                   & \multicolumn{1}{l|}{64.29}                                                                 & 63.33                                                                & 84.53                                                             & 72.41                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 66.20                                                                       & 78.95                                                                    & \multicolumn{1}{l|}{72.02}                                                                & 79.99                                                                       & 63.99                                                                   & \multicolumn{1}{l|}{71.11}                                                                 & 66.34                                                                & 78.80                                                             & 72.04                                                         \\
\multicolumn{1}{l|}{\textbf{20000}}                                                      & 66.80                                                                       & 72.70                                                                    & \multicolumn{1}{l|}{69.63}                                                                & 76.08                                                                       & 76.08                                                                   & \multicolumn{1}{l|}{76.08}                                                                 & 66.89                                                                & 72.74                                                             & 69.69                                                         \\
\multicolumn{1}{l|}{\textbf{24000}}                                                      & 64.67                                                                       & 62.67                                                                    & \multicolumn{1}{l|}{63.65}                                                                & 70.82                                                                       & 84.98                                                                   & \multicolumn{1}{l|}{77.26}                                                                 & 64.73                                                                & 62.89                                                             & 63.80                                                         \\
\multicolumn{1}{l|}{\textbf{28000}}                                                      & 57.18                                                                       & 50.16                                                                    & \multicolumn{1}{l|}{53.44}                                                                & 65.46                                                                       & 91.65                                                                   & \multicolumn{1}{l|}{76.38}                                                                 & 57.27                                                                & 50.57                                                             & 53.71                                                         \\
\multicolumn{1}{l|}{\textbf{32000}}                                                      & 48.83                                                                       & 35.77                                                                    & \multicolumn{1}{l|}{41.29}                                                                & 60.32                                                                       & 96.50                                                                   & \multicolumn{1}{l|}{74.23}                                                                 & 48.94                                                                & 36.37                                                             & 41.73                                                         \\
\multicolumn{1}{l|}{\textbf{36000}}                                                      & 30.36                                                                       & 18.83                                                                    & \multicolumn{1}{l|}{23.24}                                                                & 55.02                                                                       & 99.03                                                                   & \multicolumn{1}{l|}{70.74}                                                                 & 30.61                                                                & 19.62                                                             & 23.91                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Compute Mahalanobis Distance}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 55.01                                                                       & 87.24                                                                    & \multicolumn{1}{l|}{67.47}                                                                & 88.65                                                                       & 17.73                                                                   & \multicolumn{1}{l|}{29.55}                                                                 & 55.34                                                                & 86.55                                                             & 67.51                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 59.96                                                                       & 86.14                                                                    & \multicolumn{1}{l|}{70.70}                                                                & 86.03                                                                       & 34.41                                                                   & \multicolumn{1}{l|}{49.16}                                                                 & 60.22                                                                & 85.63                                                             & 70.71                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 65.69                                                                       & 84.49                                                                    & \multicolumn{1}{l|}{73.91}                                                                & 84.08                                                                       & 50.45                                                                   & \multicolumn{1}{l|}{63.06}                                                                 & 65.87                                                                & 84.15                                                             & 73.90                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 72.46                                                                       & 81.94                                                                    & \multicolumn{1}{l|}{76.91}                                                                & 82.09                                                                       & 65.67                                                                   & \multicolumn{1}{l|}{72.97}                                                                 & 72.56                                                                & 81.78                                                             & 76.89                                                         \\
\multicolumn{1}{l|}{\textbf{20000}}                                                      & 80.56                                                                       & 77.95                                                                    & \multicolumn{1}{l|}{79.23}                                                                & 79.88                                                                       & 79.88                                                                   & \multicolumn{1}{l|}{79.88}                                                                 & 80.56                                                                & 77.97                                                             & 79.24                                                         \\
\multicolumn{1}{l|}{\textbf{24000}}                                                      & 89.12                                                                       & 70.48                                                                    & \multicolumn{1}{l|}{78.71}                                                                & 75.97                                                                       & 91.17                                                                   & \multicolumn{1}{l|}{82.88}                                                                 & 88.99                                                                & 70.69                                                             & 78.79                                                         \\
\multicolumn{1}{l|}{\textbf{28000}}                                                      & 95.61                                                                       & 57.33                                                                    & \multicolumn{1}{l|}{71.68}                                                                & 69.62                                                                       & 97.47                                                                   & \multicolumn{1}{l|}{81.22}                                                                 & 95.35                                                                & 57.72                                                             & 71.91                                                         \\
\multicolumn{1}{l|}{\textbf{32000}}                                                      & 96.78                                                                       & 39.31                                                                    & \multicolumn{1}{l|}{55.91}                                                                & 62.08                                                                       & 99.33                                                                   & \multicolumn{1}{l|}{76.41}                                                                 & 96.44                                                                & 39.90                                                             & 56.45                                                         \\
\multicolumn{1}{l|}{\textbf{36000}}                                                      & 85.17                                                                       & 19.91                                                                    & \multicolumn{1}{l|}{32.28}                                                                & 55.51                                                                       & 99.91                                                                   & \multicolumn{1}{l|}{71.36}                                                                 & 84.88                                                                & 20.70                                                             & 33.28                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Compute Max Probability}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 52.80                                                                       & 83.88                                                                    & \multicolumn{1}{l|}{64.81}                                                                & 64.35                                                                       & 12.87                                                                   & \multicolumn{1}{l|}{21.45}                                                                 & 52.91                                                                & 83.17                                                             & 64.68                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 56.93                                                                       & 81.61                                                                    & \multicolumn{1}{l|}{67.07}                                                                & 72.09                                                                       & 28.84                                                                   & \multicolumn{1}{l|}{41.19}                                                                 & 57.08                                                                & 81.09                                                             & 67.00                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 62.75                                                                       & 80.25                                                                    & \multicolumn{1}{l|}{70.43}                                                                & 75.80                                                                       & 45.48                                                                   & \multicolumn{1}{l|}{56.85}                                                                 & 62.87                                                                & 79.91                                                             & 70.37                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 70.62                                                                       & 79.44                                                                    & \multicolumn{1}{l|}{74.77}                                                                & 78.72                                                                       & 62.98                                                                   & \multicolumn{1}{l|}{69.97}                                                                 & 70.70                                                                & 79.28                                                             & 74.74                                                         \\
\multicolumn{1}{l|}{\textbf{20000}}                                                      & 78.19                                                                       & 79.14                                                                    & \multicolumn{1}{l|}{78.66}                                                                & 80.31                                                                       & 75.32                                                                   & \multicolumn{1}{l|}{77.73}                                                                 & 78.21                                                                & 79.11                                                             & 78.66                                                         \\
\multicolumn{1}{l|}{\textbf{24000}}                                                      & 69.62                                                                       & 53.95                                                                    & \multicolumn{1}{l|}{60.79}                                                                & 63.54                                                                       & 76.25                                                                   & \multicolumn{1}{l|}{69.32}                                                                 & 69.56                                                                & 54.18                                                             & 60.91                                                         \\
\multicolumn{1}{l|}{\textbf{28000}}                                                      & 60.83                                                                       & 35.01                                                                    & \multicolumn{1}{l|}{44.44}                                                                & 55.17                                                                       & 77.24                                                                   & \multicolumn{1}{l|}{64.37}                                                                 & 60.77                                                                & 35.43                                                             & 44.76                                                         \\
\multicolumn{1}{l|}{\textbf{32000}}                                                      & 47.94                                                                       & 17.91                                                                    & \multicolumn{1}{l|}{26.08}                                                                & 49.95                                                                       & 79.92                                                                   & \multicolumn{1}{l|}{61.47}                                                                 & 47.96                                                                & 18.52                                                             & 26.72                                                         \\
\multicolumn{1}{l|}{\textbf{36000}}                                                      & 31.03                                                                       & 4.86                                                                     & \multicolumn{1}{l|}{8.40}                                                                 & 47.94                                                                       & 86.28                                                                   & \multicolumn{1}{l|}{61.63}                                                                 & 31.20                                                                & 5.67                                                              & 9.60                                                          \\ \hline
\multicolumn{10}{c}{\textbf{Placeholders Algorithm}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{l|}{\textbf{4000}}                                                       & 53.55                                                                       & 84.46                                                                    & \multicolumn{1}{l|}{65.54}                                                                & 75.40                                                                       & 15.08                                                                   & \multicolumn{1}{l|}{25.13}                                                                 & 53.76                                                                & 83.77                                                             & 65.49                                                         \\
\multicolumn{1}{l|}{\textbf{8000}}                                                       & 58.48                                                                       & 82.58                                                                    & \multicolumn{1}{l|}{68.47}                                                                & 78.90                                                                       & 31.56                                                                   & \multicolumn{1}{l|}{45.09}                                                                 & 58.68                                                                & 82.07                                                             & 68.43                                                         \\
\multicolumn{1}{l|}{\textbf{12000}}                                                      & 64.79                                                                       & 80.94                                                                    & \multicolumn{1}{l|}{71.97}                                                                & 80.14                                                                       & 48.09                                                                   & \multicolumn{1}{l|}{60.11}                                                                 & 64.95                                                                & 80.62                                                             & 71.94                                                         \\
\multicolumn{1}{l|}{\textbf{16000}}                                                      & 71.80                                                                       & 79.45                                                                    & \multicolumn{1}{l|}{75.43}                                                                & 80.50                                                                       & 64.40                                                                   & \multicolumn{1}{l|}{71.56}                                                                 & 71.89                                                                & 79.30                                                             & 75.41                                                         \\
\multicolumn{1}{l|}{\textbf{20000}}                                                      & 79.24                                                                       & 78.16                                                                    & \multicolumn{1}{l|}{78.70}                                                                & 80.21                                                                       & 77.38                                                                   & \multicolumn{1}{l|}{78.77}                                                                 & 79.25                                                                & 78.15                                                             & 78.70                                                         \\
\multicolumn{1}{l|}{\textbf{24000}}                                                      & 68.34                                                                       & 56.73                                                                    & \multicolumn{1}{l|}{62.00}                                                                & 66.17                                                                       & 79.41                                                                   & \multicolumn{1}{l|}{72.19}                                                                 & 68.32                                                                & 56.95                                                             & 62.12                                                         \\
\multicolumn{1}{l|}{\textbf{28000}}                                                      & 58.76                                                                       & 40.38                                                                    & \multicolumn{1}{l|}{47.87}                                                                & 59.16                                                                       & 82.82                                                                   & \multicolumn{1}{l|}{69.02}                                                                 & 58.76                                                                & 40.80                                                             & 48.16                                                         \\
\multicolumn{1}{l|}{\textbf{32000}}                                                      & 40.80                                                                       & 26.21                                                                    & \multicolumn{1}{l|}{31.92}                                                                & 55.09                                                                       & 88.15                                                                   & \multicolumn{1}{l|}{67.81}                                                                 & 40.94                                                                & 26.82                                                             & 32.41                                                         \\
\multicolumn{1}{l|}{\textbf{36000}}                                                      & 27.90                                                                       & 13.79                                                                    & \multicolumn{1}{l|}{18.46}                                                                & 52.67                                                                       & 94.81                                                                   & \multicolumn{1}{l|}{67.72}                                                                 & 28.15                                                                & 14.60                                                             & 19.23                                                         \\ \hline
\multicolumn{10}{c}{\textbf{Few shot Open set Recognition}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\end{tabular}
    }
    \caption{
    Novelty Detection Stage performance of Dataset 2.
    }
    \label{tab:ds2_s1}
\end{table*}

==> Tables/ds3_sample_class_detection.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}
    {
\begin{tabular}{lllllllll}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Novelties \\ Predicted\end{tabular}}} & \multicolumn{4}{l}{\textbf{\# of classes detected}}                                & \multicolumn{4}{l}{\textbf{\# of Samples detected}}           \\ \cline{2-9} 
                                                                                          & \textbf{CM} & \textbf{ED} & \textbf{MD} & \multicolumn{1}{l|}{\textbf{MP}} & \textbf{CM} & \textbf{ED} & \textbf{MD} & \textbf{MP} \\ \hline
\textbf{1000}                                                                            & 25            & 2             & 25            & \multicolumn{1}{l|}{25} & 389           & 282           & 852           & 917           \\
\textbf{2000}                                                                            & 25            & 3             & 25            & \multicolumn{1}{l|}{25} & 864           & 818           & 1687          & 1813          \\
\textbf{3000}                                                                            & 25            & 6             & 25            & \multicolumn{1}{l|}{25} & 1351          & 1499          & 2134          & 2685          \\
\textbf{4000}                                                                            & 25            & 7             & 25            & \multicolumn{1}{l|}{25} & 1873          & 2488          & 2893          & 3536          \\
\textbf{5000}                                                                            & 25            & 7             & 25            & \multicolumn{1}{l|}{25} & 2423          & 3130          & 3257          & 4369          \\
\textbf{6000}                                                                            & 25            & 8             & 25            & \multicolumn{1}{l|}{25} & 2995          & 3732          & 3476          & 5179          \\
\textbf{7000}                                                                            & 25            & 9             & 25            & \multicolumn{1}{l|}{25} & 3568          & 4090          & 3882          & 5985          \\
\textbf{8000}                                                                            & 25            & 10            & 25            & \multicolumn{1}{l|}{25} & 4164          & 4601          & 4059          & 6798          \\
\textbf{9000}                                                                            & 25            & 12            & 25            & \multicolumn{1}{l|}{25} & 4757          & 4679          & 4275          & 7600          \\
\textbf{10000}                                                                           & 25            & 12            & 25            & \multicolumn{1}{l|}{25} & 5338          & 5487          & 4451          & 8364          \\ \hline
\end{tabular}
}
\caption{
    insert caption
    }
    \label{tab_ds3}
\end{table}
